High Dimensional Quantum Eavesdropping: A Hypothetical Attack on BB84 & SSP

Quantum key distribution algorithms are considered secure because they leverage quantum phenomena to provide security. As such, eavesdroppers can be detected by analyzing the error rate in the shared key obtained by the parties performing the key exchange. Nevertheless, this paper developed and investigated a novel attack strategy capable of being undetected through error analysis of the shared key. Said attack entails an eavesdropper measuring the quantum channel (i.e., the channel used to transmit quantum particles between two parties) using a higher dimension than that used by the legitimate parties. By measuring a particle in a dimension that spans all possible states in a given quantum key distribution algorithm, the collapsed state of the measured particle should be undetectable when measured in the lower dimension. To analyze the proposed high-dimensional eavesdropping attack, the simulator Cirq was used to model the attack on BB84, a four-dimensional variant of BB84, and the Six-State Protocol. The results of these simulations show the efficiency of this attack, with an eavesdropper being undetectable through quantum bit error rate analysis in each algorithm This promotes the need for further analysis of the high-dimensional eavesdropping attack on physical hardware and other quantum key distribution algorithms

==> sections/lit-review/subsections/quantum-cloning.tex <==

\subsection{Quantum Cloning} \label{subsec:lit-review-cloning}

\gls{qkd} algorithms rely on the no-cloning theorem to provide security~\cite{Sabani2022}, which states that it is
impossible for one to perfectly copy a quantum state without altering it~\cite{Wootters1982}.
Despite this, the creation of imperfect copies of quantum states is possible using quantum cloning
machines~\cite{Idan2024, Iqbal2023}.

\citeA{Bouchard2017} explored the use of such a machine to perform a \gls{mitm} attack on
BB84 in a paper titled ``High-dimensional quantum cloning and applications to quantum hacking''.
It detailed a high-dimensional \gls{uqcm} capable of creating imperfect clones of the \gls{oam} states of photons.
Their \gls{uqcm} required two input qubits, the first qubit being the one sent between Alice and Bob, and the second
being a qubit in an even superposition between all $d$ dimensions of the first qubit.
The \gls{uqcm} was used to attack both high-dimensional and standard versions of BB84, finding that the
high-dimensional protocol made an eavesdropper's presence clearly visible and demonstrating the improved security of
\gls{hdqkd} compared to their lower dimensional variants.

